Methodology for Mining, Discovering and Analyzing Semantic Human Mobility Behaviors

Various institutes produce large semantic datasets containing information regarding daily activities and human mobility. The analysis and understanding of such data are crucial for urban planning, socio-psychology, political sciences, and epidemiology. However, none of the typical data mining processes have been customized for the thorough analysis of semantic mobility sequences to translate data into understandable behaviors. Based on an extended literature review, we propose a novel methodological pipeline called simba (Semantic Indicators for Mobility and Behavior Analysis), for mining and analyzing semantic mobility sequences to identify coherent information and human behaviors. A framework for semantic sequence mobility analysis and clustering explicability based on integrating different complementary statistical indicators and visual tools is implemented. To validate this methodology, we used a large set of real daily mobility sequences obtained from a household travel survey. Complementary knowledge is automatically discovered in the proposed method.

==> Paper/old_table.tex <==
\begin{table*}[]
\begin{tabular}{l m{3.15cm} m{5.2cm}}
\hline 
\multicolumn{1}{l}{{\scriptsize{}Techniques}} & {\scriptsize{}Forms} & {\scriptsize{}Description}\tabularnewline
\hline 
\hline 
\multicolumn{3}{c}{{\scriptsize{}\textit{Frequency distribution}}} \\
\hline 
{\scriptsize{}Length distribution} & {\scriptsize{}$\forall X\in\mathcal{D},|X|$} & {\scriptsize{}Frequency distribution of sequences' length $|X|$ in the dataset
$\mathcal{D}$. }\tabularnewline
{\scriptsize{}State distribution} & {\scriptsize{}$\forall x\in\Sigma,\underset{X\in\mathcal{D}}{\sum}f(x)$} & {\scriptsize{}Frequency distribution for each symbol $x$
in dataset $\mathcal{D}$.}
\tabularnewline
\hline 
\multicolumn{3}{c}{{\scriptsize{}\textit{Transition}}} \\
\hline 
\multicolumn{1}{l}{{\scriptsize{}OD matrix}} & {\scriptsize{}$t_{ij}=\underset{X\in\mathcal{D}}{\sum}f(x_{i}\rightarrow x_{j})$} & {\scriptsize{}Origin-Destination (OD) matrix $T$ where $t_{ij}$
is the number of transition from state $x_{i}$ to $x_{j}$. }\tabularnewline
\multicolumn{1}{l}{{\scriptsize{}Daily patterns}} & {\scriptsize{}$G=(V,E)$ with $V=\{x|x\in X\}$ and $E=\left\{ (x_{i},x_{i+1})|i\in [\![ 1,n-1]\!] \right\} $} & {\scriptsize{}Network i.e. graph representation $G$ of a given sequence
$X$. Each edge $(x_{i},x_{j})$ represent the transition from $x_{i}$
to $x_{j}$. }\tabularnewline
\hline 
\multicolumn{3}{c}{{\scriptsize{}\textit{Entropy}}} \\
\hline 
{\scriptsize{}Real entropy} & {\scriptsize{}$-\underset{X'\subset X}{\sum}p(X')\log_{2}p(X')$} & {\scriptsize{}Real entropy of a sequence. $p(X')$ is the probability
of finding a particular subsequence $X'$ in $X$.}\tabularnewline
{\scriptsize{}Distinct symbols} & {\scriptsize{}$\delta(X)$} & {\scriptsize{}Number of distinct symbols in sequence $X$.}\tabularnewline
{\scriptsize{}Regularity} & {\scriptsize{}$\frac{|X|}{\delta(X)}$} & {\scriptsize{}Ratio between the length of the sequence $|X|$ and
the number of unique symbols $\delta(X)$ in it.}\tabularnewline
{\scriptsize{}Stationarity} & {\scriptsize{}$\frac{1}{n}\stackrel[i=1]{n}{\sum}\tau(x_{i})$} & {\scriptsize{}Mean duration for which the person stays
continuously in the same state. $\tau(x_i)$ denotes the duration spend for state $x_i$.}
\tabularnewline
\hline 
\multicolumn{3}{c}{{\scriptsize{}\textit{Centrality}}} \\
\hline 
{\scriptsize{}Medoid element} & {\scriptsize{}$\underset{X\in\mathcal{D}}{\text{argmin}}\left\{ \underset{Y\in\mathcal{D}}{\sum}d(X,Y)\right\} $} & {\scriptsize{}Element which minimizes the distance $d$ to all elements
in the dataset.}\tabularnewline
{\scriptsize{}Mode element} & {\scriptsize{}$\underset{X\in\mathcal{D}}{\text{argmax}}\left\{ f(X)\right\} $} & {\scriptsize{}Element with the highest frequency $f$ in the dataset.}\tabularnewline
\hline 
\multicolumn{3}{c}{{\scriptsize{}\textit{Scattering and outliers}}} \\
\hline 
{\scriptsize{}Diameter elements} & {\scriptsize{}$\underset{X,Y\in\mathcal{D}}{\text{argmax}}\left\{ d(X,Y)\right\} $} & {\scriptsize{}Most extreme elements in the dataset which maximize the distance.}\tabularnewline
{\scriptsize{}Distance distribution} & {\scriptsize{}$\forall X, Y\in\mathcal{D},d(X,Y)$} & {\scriptsize{}Distribution of the distance between all couple of sequences $X,Y$ in the dataset or subset e.g. cluster.}\tabularnewline
{\scriptsize{}Silhouette} & {\scriptsize{} $s(X) = \frac{b(X)-a(X)}{\max\{a(X), b(X)\}}$ and 

$Sil(C_i) = \frac{1}{|C_i|}\underset{X\in C_i}{\sum} s(X)$} & {\scriptsize{} Let $(C_1, ..., C_k) $ a partition of $\mathcal{D}$. Value which quantifies how $X\in C_i$ is appropriately clustered. Where:
\begin{itemize}
    \item $a(X) = \frac{1}{|C_i|-1}\underset{Y\in C_i,Y\neq X}{\sum}d(X,Y)$
    \item $b(X)=\underset{C_j\neq C_i}{\min}\frac{1}{|C_j|}\underset{Y\in C_j}{\sum}d(X,Y)$
\end{itemize}
Quality index of a clustering. 
}
\tabularnewline
\hline 
\multicolumn{3}{c}{{\scriptsize{}\textit{Logic rules}}} \\
\hline 
\multicolumn{1}{l}{{\scriptsize{}Decision rules}} & {\scriptsize{}$r_{1}\wedge r_{2}\wedge...\wedge r_{n}\Rightarrow C$} & {\scriptsize{}Rules to describe a subset $C$  of data extracted e.g. cluster from a decision
tree or association rule learning algorithm. }\tabularnewline
\hline 
\end{tabular}{\scriptsize \par}
\end{table*}

==> Paper/tab_mesures.tex <==
{\scriptsize{}}%
\begin{table*}
\caption{Description of main similarity measures for semantic sequences}
\label{tab:description}  
\begin{tabular}{m{2.2cm}ccm{5.5cm}}
\hline 
\multirow{2}{*}{{\scriptsize{}Measure}} & \multicolumn{2}{c}{{\scriptsize{}Type}} & \multirow{2}{*}{{\scriptsize{}Description}}\tabularnewline
\cline{2-3} 
 & {\scriptsize{}Match} & {\scriptsize{}Edit.} & \tabularnewline
\hline 
{\scriptsize{}MSM \cite{Furtado16}, SMSM \cite{Lehmann19}} & {\scriptsize{}$\times$} &  & {\scriptsize{}Agregation of maching functions of each dimension.}\tabularnewline
{\scriptsize{}SVRspell \cite{Elzinga15}} & {\scriptsize{}$\times$} &  & {\scriptsize{}Based on number of matching spell subsequences with
spell length weights.}\tabularnewline
{\scriptsize{}Jiang et al. \cite{Jiang12}} & {\scriptsize{}$\times$} &  & {\scriptsize{}Euclidean distance between appropriate eigen activities.}\tabularnewline
{\scriptsize{}Hamming} & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} & {\scriptsize{}Number of mismatches.}\tabularnewline
{\scriptsize{}\ \ Generalized } &  & {\scriptsize{}$\times$} & {\scriptsize{}Sum of mismatches with similarity between elements.}\tabularnewline
{\scriptsize{}DHD \cite{Lesnard10}} &  & {\scriptsize{}$\times$} & {\scriptsize{}Sum of mismatches with positionwise state-dependent
weights.}\tabularnewline
{\scriptsize{}Levenshtein, OM, LCSS} & \multirow{1}{*}{} & \multirow{1}{*}{{\scriptsize{}$\times$}} & \multirow{1}{*}{{\scriptsize{}Number of edit operations to turn $S_{1}$ into $S_{2}$.}}\tabularnewline
{\scriptsize{}\ \ Generalized } &  & {\scriptsize{}$\times$} & {\scriptsize{}Sum of edit costs to turn $S_{1}$ into $S_{2}$.}\tabularnewline
{\scriptsize{}CED \cite{Moreau19b}} &  & {\scriptsize{}$\times$} & {\scriptsize{}OM with costs weighted by edit position and symbols
nearby.}\tabularnewline
{\scriptsize{}Trate (TDA) \cite{Rohwer05}} &  & {\scriptsize{}$\times$} & {\scriptsize{}OM with costs based on transition rates.}\tabularnewline
{\scriptsize{}OMSlen \cite{Halpin10}} &  & {\scriptsize{}$\times$} & {\scriptsize{}OM with costs weighted by spell length.}\tabularnewline
\hline 
\end{tabular}{\scriptsize \par}
\end{table*}  


%%%

\begin{table*}
\caption{Properties of main similarity measures for semantic sequences}
\label{tab:properties} 

{\scriptsize{}}%
\begin{tabular}{m{2.2cm}ccccccc}
\hline 
\multirow{2}{*}{{\scriptsize{}Measure}} & \multicolumn{7}{c}{{\scriptsize{}Properties}}\tabularnewline
\cline{2-8} 
 & {\scriptsize{}Metric} & {\scriptsize{}T. warp} & {\scriptsize{}Ctxt} & {\scriptsize{}Permut.} & {\scriptsize{}Spell} & {\scriptsize{}Sim.} & {\scriptsize{}Multi. dim}\tabularnewline
\hline 
{\scriptsize{}MSM \cite{Furtado16}, SMSM \cite{Lehmann19}} &  & {\scriptsize{}$\times$} &  &  &  &  & {\scriptsize{}$\times$}\tabularnewline
{\scriptsize{}SVRspell \cite{Elzinga15}} & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} &  & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} & \tabularnewline
{\scriptsize{}Jiang et al. \cite{Jiang12}} & {\scriptsize{}$\times$} &  &  &  &  &  & \tabularnewline
{\scriptsize{}Hamming} & {\scriptsize{}$\times$} &  &  &  &  &  & \tabularnewline
{\scriptsize{}\ \ Generalized } & {\scriptsize{}$\times^{\dagger}$} &  &  &  &  & {\scriptsize{}$\times$} & \tabularnewline
{\scriptsize{}DHD \cite{Lesnard10}} &  &  & {\scriptsize{}$\times$} &  &  & {\scriptsize{}$\times$} & \tabularnewline
{\scriptsize{}Levenshtein, OM, LCSS} & \multirow{1}{*}{{\scriptsize{}$\times$}} & \multirow{1}{*}{{\scriptsize{}$\times$}} & \multirow{1}{*}{} & \multirow{1}{*}{} & \multirow{1}{*}{} & \multirow{1}{*}{} & \multirow{1}{*}{}\tabularnewline
{\scriptsize{}\ \ Generalized } & {\scriptsize{}$\times^{\dagger}$} & {\scriptsize{}$\times$} &  &  &  & {\scriptsize{}$\times$} & \tabularnewline
{\scriptsize{}CED \cite{Moreau19b}} & {\scriptsize{}$\times^{\dagger}$} & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} & \tabularnewline
{\scriptsize{}Trate (TDA) \cite{Rohwer05}} &  & {\scriptsize{}$\times$} &  &  &  & {\scriptsize{}$\times$} & \tabularnewline
{\scriptsize{}OMSlen \cite{Halpin10}} & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} & {\scriptsize{}$\times$} &  & {\scriptsize{}$\times$} &  & \tabularnewline
\hline \tabularnewline
\multicolumn{8}{l}{{\scriptsize{}$\dagger$ Depends if costs fulfil the triangle inequality and/or parameters.}}

\end{tabular}{\scriptsize \par}

\end{table*}


\begin{table*}
\caption{Complexity and parameters of main similarity measures for semantic sequences}
\label{tab:complexity} 
{\scriptsize{}}%
\begin{tabular}{m{2.2cm}cccm{2.7cm}}
\hline 
\multirow{2}{*}{{\scriptsize{}Measure}} & \multirow{2}{*}{{\scriptsize{}Complexity}} & \multicolumn{3}{c}{{\scriptsize{}Parameters}}\tabularnewline
\cline{3-5} 
 &  & {\scriptsize{}Subs} & {\scriptsize{}Indels} & {\scriptsize{}Other}\tabularnewline
\hline 
{\scriptsize{}MSM \cite{Furtado16}, SMSM \cite{Lehmann19}} & {\scriptsize{}$O(n\times p)$} &  &  & {\scriptsize{}Set of distances $\mathcal{D}$; weight vector $w$; threshold vector $maxDist$}\tabularnewline
{\scriptsize{}SVRspell \cite{Elzinga15}} & {\scriptsize{}$O\left(|\Sigma|^{\max(n,p)}\right)$} &  &  & {\scriptsize{}Subsequence length weight $a$; spell duration weight
$b$}\tabularnewline
{\scriptsize{}Jiang et al. \cite{Jiang12}} & {\scriptsize{}$O(n\times p)$} &  &  & {\scriptsize{}Number of activities}\tabularnewline
{\scriptsize{}Hamming} & {\scriptsize{}$O(n)$} &  &  & \tabularnewline
{\scriptsize{}\ \ Generalized } & {\scriptsize{}$O(n)$} & {\scriptsize{}User} &  & \tabularnewline
{\scriptsize{}DHD \cite{Lesnard10}} & {\scriptsize{}$O(n)$} & {\scriptsize{}Data} &  & \tabularnewline
{\scriptsize{}Levenshtein, OM, LCSS} & \multirow{1}{*}{{\scriptsize{}$O(n\times p)$}} & \multirow{1}{*}{{\scriptsize{}Single}} & \multirow{1}{*}{{\scriptsize{}Single}} & \multirow{1}{*}{}\tabularnewline
{\scriptsize{}\ \ Generalized } & {\scriptsize{}$O(n\times p)$} & {\scriptsize{}User} & {\scriptsize{}Single} & \tabularnewline
{\scriptsize{}CED \cite{Moreau19b}} & {\scriptsize{}$O(n\times p\times\max(n,p))$} & {\scriptsize{}Ontology} & {\scriptsize{}Auto} & {\scriptsize{}Ontology; Context function $f_{k}$; Context weight
$\alpha$}\tabularnewline
{\scriptsize{}Trate (TDA) \cite{Rohwer05}} & {\scriptsize{}$O(n\times p)$} & {\scriptsize{}Data} & {\scriptsize{}Single} & {\scriptsize{}Transition lag $q$}\tabularnewline
{\scriptsize{}OMSlen \cite{Halpin10}} & {\scriptsize{}$O(n\times p)$} & {\scriptsize{}User} & {\scriptsize{}Multiple} & {\scriptsize{}Spell length weight $h$}\tabularnewline
\hline 
\end{tabular}{\scriptsize \par}
\end{table*}
